Single Point Transductive Prediction

Standard methods in supervised learning separate training and prediction: the model is fit independently of any test points it may encounter. However, can knowledge of the next test point $\mathbf{x}_{\star}$ be exploited to improve prediction accuracy? We address this question in the context of linear prediction, showing how techniques from semi-parametric inference can be used transductively to combat regularization bias. We first lower bound the $\mathbf{x}_{\star}$ prediction error of ridge regression and the Lasso, showing that they must incur significant bias in certain test directions. We then provide non-asymptotic upper bounds on the $\mathbf{x}_{\star}$ prediction error of two transductive prediction rules. We conclude by showing the efficacy of our methods on both synthetic and real data, highlighting the improvements single point transductive prediction can provide in settings with distribution shift.

==> prelims.tex <==
\textbf{Notation and Assumptions:}
We will use bolded letters (i.e. $\bx$) to refer to vectors and capitalized and bolded letters to refer to matrices (i.e. $\bX$). We use $[p]$ for set $\{1, \hdots, p \}$ and $\Vert \bbeta_0 \Vert_0$ to for the number of non-zero elements in $\bbeta_0$; $S \subset [p]$ denotes the subset of indices on which $\bbeta_0$ is supported. Generically, "hatted" vectors, such as $\hat{\bbeta}$ refer to a estimator of $\bbeta_0$. We define the standard Lasso estimator as $\hat{\bbeta}_{L} = \arg \min_{\bbeta} \frac{1}{2n} \normt{\by - \bX \bbeta}^2 + \lambda \normo{\bbeta}$.
\\
We now detail some important assumptions which are standard throughout the literature on high-dimensional inference.
\begin{assumption} (Model is Well-Specified)
  The data $(\bY, \bX)$ is generated from the model in \eq{model}.
  \label{assump:well_spec}
\end{assumption}

\begin{assumption} (Bounded Covariance)
In the random design setting (where covariates $\bx_i$ are random),
  their population covariance $\bSigma$ satisfies $\bSigma_{ii} \leq 1/2$, $\sigma_{\max}(\bSigma) \leq C_{\max}$ and $\sigma_{\min}(\bSigma) \geq C_{\min}$. \label{assump:cov}
\end{assumption}

\begin{assumption} (sub-Gaussian Design)
  The vector of covariates $\bSigma^{-1/2} \bx$ is a sub-Gaussian random vector with parameter $\kappa \geq 1$, in the sense that,
  \begin{talign}
      \E[\exp(\bv^\top \bx)] \leq \exp \left( \frac{\kappa^2 \Vert \bSigma^{1/2} \bv \Vert^2}{2} \right)
  \end{talign}
  \label{assump:design}
\end{assumption}

\begin{assumption} (sub-Gaussian Noise)
  The noise $\bepsilon$ is sub-Gaussian with parameter $\sigma^2$ and independent of $\bX$.
  \label{assump:noise1}
\end{assumption}
Our principal goal in this paper will be to understand prediction risk of an estimator $\hat{\bbeta}(\by, \bX)$ on a new test datapoint $\xstar$, 
$
    \mathcal{R}_p(\xstar, \hat{\bbeta}) = \E[(\ystar-\langle \xstar, \hat{\bbeta} \rangle)^2] = \sigma^2 + \E[(\langle \xstar, \hat{\bbeta}-\bbeta_0 \rangle)^2]
$
where $\ystar = \xstar^\top \bbeta_0+ \epsilon$. As the additive noise $\sigma^2$ is irreducible, for any estimator we focus our study on  $\E[(\langle \xstar, \hat{\bbeta}-\bbeta_0 \rangle)^2]$. 
To accommodate non-stationary learning settings, we do not impose any distributional assumptions on $\bx_*$; in particular it need not be drawn from the training distribution.

The proofs of all results in this paper are deferred to the Appendix.

==> transduction_review.tex <==
\section{Review of Papers on Transductive Prediction}

The transductive lasso (TDL) \citep{alquier2012transductive}. The TDL method in [1] provides an identical error bound to that of Lasso with only the restricted-eigenvalue constant (RE constant) potentially improved by transduction. Their result, unlike our Thm. BLAH, does not eliminate the dimension-dependent bias of the Lasso to provide O(1/n) rates and also does not guarantee that RE-like constant is always improved.  \notate{Can we be more precise here?  Can we say something like under the conditions of our Corollary 3, the prediction error of TDL is still $\Omega(\trimmednorm{\xstar}{s}^2  \frac{\sigma_{\epsilon}^2 \log p}{n})$, just like the Lasso?} \nnote{One point that makes their results a bit more difficult to parse is that all all results are under fixed design. The complication here is that their method uses a "preliminary" estimator to do the transductive labeling -- so I think the efficiency of their estimator will always depend on this and its not immediately clear how to apply the same lower bound since their is dependence between the two stages.}

transductive ridge regression (TDRR) \citep{chapelle2000transductive}. The work of [2] presents a uniform convergence, VC-based bound which upper bounds the transductive risk by the empirical risk plus an additional, positive term depending on the hypothesis class, the number of datapoints, and other problem-dependent parameters. This bound does not imply that transduction can improve prediction in the single-point setting with respect to a prediction rule found via empirical risk minimization. Moreover, the generalization guarantees are not instantiated/applied to the TDKNN algorithm used in their experiments. \notate{is it fair to say that the final term in the error bound is only small when the number of unlabeled test points is large?} \nnote{I think the error term can be made small as the number of training points in the empirical risk goes to zero. I think the main thing is when number of test points is small, its not clear this bound is ever better then whatever u could guarantee doing normal ERM; although another difference here is they are not interested in minimizing population risk here but transductive risk.} 

Transductive ridge regression with kernel-nearest neighbor labelling (LTR) is proposed in \citep{cortes2007transductive} for which stability-based guarantees are provided in \citet{cortes2008stability}; however the error bound on the transductive risk by empirical risk plus an additive error is only guaranteed to be small when the number of unlabeled test points is large. \notate{should discuss whether the other cortes paper has guarantees}



\notate{Need to add Bellec}
\nnote{This is in current related work}

\notate{Should add original Vapnik paper}
\citet{vapnik1998statistical}

\notate{Should add other paper that cortes compares to in their work}

\citet{belkin2006manifold} presents a framework for transduction and SSL using a form of manifold learning.
  
